Exploring metallicity-dependent rates of Type Ia supernovae and their impact on galaxy formation

Type Ia supernovae play a critical role in stellar feedback and elemental enrichment in galaxies. Recent transient surveys like the All-Sky Automated Survey for Supernova (ASAS-SN) and the Dark Energy Survey (DES) find that the specific Ia rate at z ~ 0 may be ~ 15-50 times higher in lower-mass galaxies than at Milky Way-mass. Independently, Milky Way observations show that the close-binary fraction of solar-type stars is higher at lower metallicity. Motivated by these observations, we use the FIRE-2 cosmological zoom-in simulations to explore the impact of varying Ia rate models, including metallicity dependence, on galaxies across a range of stellar masses: 10^7 Msun - 10^{11} Msun. First, we benchmark our simulated star-formation histories (SFHs) against observations. We show that assumed SFHs and stellar mass functions play a major role in determining the degree of tension between observations and metallicity-independent Ia rate models, and potentially cause ASAS-SN and DES observations to be much more consistent with each other than might naively appear. Models in which the Ia rate increases with decreasing metallicity (as ~ Z^{-0.5} to Z^{-1}) provide significantly better agreement with observations. Encouragingly, these increases in Ia rate (> 10 times in low-mass galaxies) do not significantly impact galaxy stellar masses and morphologies: effective radii, axis ratios, and v/sigma remain largely unaffected except for our most extreme rate models. We explore implications for both [Fe/H] and [alpha/Fe] enrichment: metallicity-dependent Ia rate models can improve agreement with observed stellar mass-metallicity relations in low-mass galaxies. Our results demonstrate that a wide range of metallicity-dependent Ia models are viable for galaxy formation and motivate future work in this area.

==> acronym_list.tex <==
\begin{acronym}
\newacro{MW}{Milky Way}
\newacro{GMC}{giant molecular clouds}
\newacro{LG}{Local Group}
\newacro{SN}{supernova}
\newacro{MDF}{metallicity distribution function}
\newacro{ISM}{interstellar medium}
\newacro{FIRE}{Feedback In Realistic Environments}
\newacro{DM}{Dark Matter}
\newacro{MFM}{Meshless Finite Mass}
\newacro{AMR}{adaptive mesh refinement}
\end{acronym}
